Interaction-Grounded Learning

Consider a prosthetic arm, learning to adapt to its user's control signals. We propose Interaction-Grounded Learning for this novel setting, in which a learner's goal is to interact with the environment with no grounding or explicit reward to optimize its policies. Such a problem evades common RL solutions which require an explicit reward. The learning agent observes a multidimensional context vector, takes an action, and then observes a multidimensional feedback vector. This multidimensional feedback vector has no explicit reward information. In order to succeed, the algorithm must learn how to evaluate the feedback vector to discover a latent reward signal, with which it can ground its policies without supervision. We show that in an Interaction-Grounded Learning setting, with certain natural assumptions, a learner can discover the latent reward and ground its policy for successful interaction. We provide theoretical guarantees and a proof-of-concept empirical evaluation to demonstrate the effectiveness of our proposed approach.

==> sections/lowerbound_old.tex <==
\section{Failure of Unsupervised Learning in IGL}
\label{sec:failunsup}

Unsupervised learning provides another approach to Interaction-Grounded Learning. If unsupervised learning distinguishes the feedback vectors generated from different rewards, then learning the optimal policy for IGL is still possible.  Indeed, the task from section~\ref{sec:experiments}  can be solved by clustering the feedback vectors.  However, in this section, we show the information-theoretical hardness of using unsupervised learning in IGL in general. 

Consider the following two environments based on the MNIST environment introduced in Section \ref{sec:experiments}. Both of these environments have the same context-action-reward setting as described in Section \ref{sec:experiments} while differing  in the feedback vector generation process.
\begin{enumerate}[topsep=1pt,parsep=1pt,itemsep=1pt,partopsep=1pt,leftmargin=1.25em]
\item[] \hspace{-1.5em} {\bf \em ENV (1).} In the first case, the feedback vector is generated according to,
\begin{align}
y|_{r = 0} = &~ \left\{ \begin{array}{lr}
\text{a random image with label ``0''},&~p = \nicefrac{8}{9};  \\
\text{a random image with label ``1''}, &~p = \nicefrac{1}{9}. 
\end{array} 
\right.
\\
y|_{r = 1} = &~ \text{a random image with label ``2'', w.p.~1}.
\end{align}
\item[] \hspace{-1.5em} {\bf \em ENV (2).}  In the second case, we exchange the images with the label ``1'' and ``2'' in the feedback vector generating process, that is,
\begin{align}
y|_{r = 0} = &~ \left\{ \begin{array}{lr}
\text{a random image with label ``0''},&~p = \nicefrac{8}{9};  \\
\text{a random image with label ``2''},&~p = \nicefrac{1}{9}. 
\end{array} 
\right.
\\
y|_{r = 1} = &~ \text{a random image with label ``1'', w.p.~1}.
\end{align}
\end{enumerate}

If the data gathering policy is the uniform policy over 10 actions, then the distribution of $y$ is \emph{identical} for the two environments above. Therefore, it is impossible to decode the exact reward of both of these two environments simultaneously only using the information from $y$. Note that this ambiguity is an information-theoretical hardness and applies to any unsupervised learning algorithm.

\begin{table}[ht]
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{cc}
\hline
\textbf{Env (1)} & \textbf{Policy Accuracy (\%)} \\ \hline
CB + KMeans      & 6.51 $\pm$ 2.11               \\
\algoname          & 80.96 $\pm$ 5.33      \\ \hline \hline
\textbf{Env (2)} & \textbf{Policy Accuracy (\%)} \\ \hline
CB + KMeans      & 83.16 $\pm$ 5.44              \\
\algoname          & 83.41 $\pm$ 4.14      \\ \hline
\end{tabular}
% }
\caption{Comparing {\algoname} with unsupervised learning methods in ENV (1) and ENV (2) introduced at the beginning of Section \ref{sec:failunsup}.}
\label{tb:mnist_cbu}
\end{table}

We also demonstrate that ambiguity by applying an imbalanced K-Means%
\footnote{The original K-Means is designed for clustering with even cluster sizes. We modify it for imbalanced K-Means in order to fit our environments.}
%
reward decoder with {\sf CB}. Table \ref{tb:mnist_cbu} shows that {\sf CB} with imbalanced K-Means indeed performs well in just one of these two environments, since there is no difference between ENV (1) and ENV (2) for the imbalanced K-Means procedure. \algoname is able to succeed in both environments.
